On Maximizing Weighted Algebraic Connectivity for Synthesizing Robust Networks

This article deals with the following simpler version of an open problem in system realization theory which has several important engineering applications: Given a collection of masses and a set of linear springs with a specified cost and stiffness, a resource constraint in terms of a budget on the total cost, the problem is to determine an optimal connection of masses and springs so that the resulting structure is as stiff as possible, i.e., the structure is connected and its smallest non-zero natural frequency is as large as possible. In this article, algebraic connectivity, or its mechanical analog - the smallest non-zero natural frequency of a connected structure was chosen as a performance objective. Algebraic connectivity determines the convergence rate of consensus protocols and error attenuation in Unmanned Aerial Vehicle (UAV) formations and is chosen to be a performance objective as it can be viewed as a measure of robustness in UAV communication networks to random node failures. Underlying the mechanical and UAV network synthesis problems is a Mixed Integer Semi-Definite Program (MISDP), an NP-hard problem. The novel contributions of this article lies in developing efficient algorithms to solve the MISDPs based on iterative primal-dual algorithm, cutting-plane methods for polyhedral outer-approximation, capturing the feasible set of MISDPs using Fiedler vectors or Laplacian with equivalency guarantees, and efficient neighborhood-search-based heuristic algorithms.

==> Chapters/acknowledgements.tex <==
%!TEX root = ../tamuthesis.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  New template code for TAMU Theses and Dissertations starting Fall 2012.  
%  For more info about this template or the 
%  TAMU LaTeX User's Group, see http://www.howdy.me/.
%
%  Author: Wendy Lynn Turner 
%	 Version 1.0 
%  Last updated 8/5/2012
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                           ACKNOWLEDGEMENTS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter*{ACKNOWLEDGEMENTS}
\addcontentsline{toc}{chapter}{ACKNOWLEDGEMENTS}  % Needs to be set to part, so the TOC doesnt add 'CHAPTER ' prefix in the TOC.
\indent 
As a graduate student at Texas A\&M University, it has been a very 
exciting journey through times that sometimes have been highly 
rewarding and other times that have been difficult but certainly 
``different'' from what I expected when I came in.
However, looking back at the wonderful seven years I spent in TAMU, I am grateful 
for the support, encouragement, and friendship of a large number of
people who have made my stay very productive and enjoyable.

First and foremost, I am deeply thankful to my thesis advisor, Dr.Swaroop Darbha,
for the opportunity to be a member of
his research group, and the freedom to grow as a researcher. He
has always been a source of inspiration with his intuition and insight, and being part of his
group has allowed me to interact with, and learn from, a number of knowledgeable
and talented individuals. I am fortunate to have been his student and thank him for the countless
hours that he has patiently spent trying to mold me into a better researcher, writer, and person.

I am also thankful to Dr.Sivakumar Rathinam for having served as a co-advisor
on my thesis committee. Having chosen a topic of research which 
was of great theoretical significance but with little literature available 
on the practical aspects, many insightful discussions with Dr.Rathinam 
helped us greatly demystify the difficulties 
associated with the understanding of the problem.

I extend my deep sense of gratitude to Dr.K.R.Rajagopal, 
Distinguished Professor of Mechanical Engineering, 
for serving on my thesis committee. If not for my frequent interactions with him regarding
the importance of research and general philosophy about learning
during my stint as a masters student, I would not have taken the audacious decision
to quit a lucrative job in the energy industry and pursue my 
doctoral studies at TAMU.

I also thank Dr.Sergiy Butenko for being a valuable member
of my thesis committee, and Dr.Kalyanababu Nakshatrala, who 
taught me a great deal about computational methods. 

I thank the many current and past members of the research group 
with whom I have had fruitful interactions. Some of them include Kaarthik Sundar, 
Satyanarayana Gupta, Myoungkuk Park and Navid Mohsenizadeh. I specially thank 
Kaarthik for spending countless hours discussing 
various open problems in combinatorial optimization and also for helping me cross my 
initial learning curve in \texttt{C++} during the starting days of my PhD.

Special thanks to my roommate, Dr.Shriram Srinivasan, for 
supporting my extra-curricular interests and putting up with my 
little idiosyncrasies at times.


I am fortunate to have spent a great deal of time with some of the very 
knowledgable and nicest faculty members at TAMU. Though 
there are many such professors, I am particularly grateful to 
Dr.N.Sivakumar (Mathematics), Dr.Shankar Bhattacharyya (Electrical Engineering), Dr.Mysore Mohan (Chemistry) and
Dr.Krishna Narayanan (Electrical Engineering). Special thanks to Dr.Bhattacharyya for 
letting me stay at one of his properties - free of cost - when I did not have any
financial support. 

I am also blessed to have formed many friendships at TAMU that have 
immensely helped me explore my interests outside work. 
Life at College station would have been very dull and much less fun without the wonderful Carnatic music 
sessions and SPICMACAY concerts. I have greatly enjoyed the weekend 
music sessions with Bhavana Iyer, Sriranjani Darbha, Srinidhi Narayanan, Aditya Nandakumar, Hariharan Bhagavatheeswaran, 
Vibhuti Chandra, Dr.N.Sivakumar, Karthik Krishnamurthy, Jagannath Vijayan, Adithya Ganapathi and Dr.Krishnakumar Ravikumar. 
Special thanks to Dr.Srikrishna Doraiswamy (also coffee mate at the lab) 
and Dr.Atul Narayan for being fine connoisseurs of Carnatic music 
and supporting our music sessions, and to Jayavel Arumugam, a good friend and
a remarkable photographer. Thanks to the families of Dr.Swaroop Darbha, 
Dr.Krishna Narayanan, Dr.Srividya Ramasubramaniam and Dr.Pazhaniappan for their sustained support in hosting 
many music sessions followed by fine food. Dr.Krishna Narayanan's family needs a special mention for hosting my concerts regularly,
turning this event into an ``Aggie'' tradition.
It would be rather incomplete to think of my progress in the field of Indian classical music without 
all my revered \emph{gurus} since my childhood. My humble salutations to Shri.T.K.V.Ramanujacharyulu,
a top notch violinist from India, for patiently teaching me the nuances of 
Carnatic music through live and Skype sessions.  

During my undergraduate studies at NIT Trichy, I was very lucky to have interacted 
with many wonderful friends and faculty members. Thanks to Dr.Hemalatha Thiagarajan
for being an excellent Mathematics professor from whom I learnt a lot. 
Special thanks to Dr.A.R.Ganesan's family for accommodating my music practice sessions on a daily basis 
for the entire four years. Thanks to G.S.Sundar Rajan, Ganapathy Ramanthan and Trichy Krishnaswamy 
for being wonderful friends and making my stay in Trichy such a memorable one. 

Finally, I thank a special group of people who are the real reasons for my continued
good fortune: my parents, Shri.S.Nagarajan and Smt.Usha Rajan, my uncle Shri.M.N.Gururaj, and my
brother Adarsh Nagarajan.  Any success of mine would be impossible without their 
unconditional love and support.

%	\pagebreak{}


==> Chapters/lists.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  New template code for TAMU Theses and Dissertations starting Fall 2012.  
%  For more info about this template or the 
%  TAMU LaTeX User's Group, see http://www.howdy.me/.
%
%  Author: Wendy Lynn Turner 
%	 Version 1.4
%  Last updated 1/27/2013
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%       TABLE OF CONTENTS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% single-space sections in Table of Contents
\renewcommand{\cftsecafterpnum}{\vskip0.5\baselineskip}
\renewcommand{\cftsubsecafterpnum}{\vskip0.5\baselineskip}
\renewcommand{\cftsubsubsecafterpnum}{\vskip0.5\baselineskip}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\phantomsection
\addcontentsline{toc}{chapter}{TABLE OF CONTENTS}  

\begin{singlespace}
\renewcommand\contentsname{\normalfont} {\centerline{TABLE OF CONTENTS}}

%\setcounter{tocdepth}{4} % This puts \subsubsection[]{×} in your List of Tables.  The default is 3.


%%%%%%%%%%%%%  Adds Page above the page number in TOC
\setlength{\cftaftertoctitleskip}{1em}
\renewcommand{\cftaftertoctitle}{%
\hfill{\normalfont {Page}\par}}



\tableofcontents

\end{singlespace}

\pagebreak{}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                           LIST OF FIGURES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\phantomsection
\addcontentsline{toc}{chapter}{LIST OF FIGURES}  

\renewcommand{\cftloftitlefont}{\center\normalfont\MakeUppercase}

\setlength{\cftbeforeloftitleskip}{-12pt} %% Positions the LOF title vertically to match the chapter titles
\renewcommand{\cftafterloftitleskip}{12pt}


\renewcommand{\cftafterloftitle}{%
\\[4em]\mbox{}\hspace{2pt}FIGURE\hfill{\normalfont Page}\vskip\baselineskip}

\begingroup


\begin{center}
\begin{singlespace}
%% These values make the lof table entries appear double spaced between.
\setlength{\cftbeforechapskip}{0.4cm}
\setlength{\cftbeforesecskip}{0.30cm}
\setlength{\cftbeforesubsecskip}{0.30cm}
\setlength{\cftbeforefigskip}{0.4cm}
\setlength{\cftbeforetabskip}{0.4cm} 

\listoffigures

\end{singlespace}
\end{center}

\pagebreak{}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                           lIST OF TABLES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\phantomsection
\addcontentsline{toc}{chapter}{LIST OF TABLES}  

\renewcommand{\cftlottitlefont}{\center\normalfont\MakeUppercase}

\setlength{\cftbeforelottitleskip}{-12pt} %% Positions the LOT title vertically to match the chapter titles

\renewcommand{\cftafterlottitleskip}{12pt}


\renewcommand{\cftafterlottitle}{%
\\[4em]\mbox{}\hspace{4pt}TABLE\hfill{\normalfont Page}\vskip\baselineskip}

\begin{center}
\begin{singlespace}

%% These values make the lot table entries appear double spaced between.
\setlength{\cftbeforechapskip}{0.4cm}
\setlength{\cftbeforesecskip}{0.30cm}
\setlength{\cftbeforesubsecskip}{0.30cm}
\setlength{\cftbeforefigskip}{0.4cm}
\setlength{\cftbeforetabskip}{0.4cm}

\listoftables 

\end{singlespace}
\end{center}
\endgroup
\pagebreak{}  % Need this for the pagenumbering to be correct. 
